Integrable systems: From the ice rule to supersymmetric fishnet Feynman diagrams

This thesis examines the correspondence between models of statistical physics and Feynman graphs of quantum field theories (QFTs) by a common property: integrability. We review integrable structures for periodic boundary conditions on both sides, while focusing on the eight- and six-vertex model and the bi-scalar fishnet theory. The latter is a double-scaled $\gamma$-deformation of $\mathcal{N} = 4$ super Yang-Mills theory. Interesting applications of integrability existing in the literature that we reconsider are the computation of the free energy in the thermodynamic limit and its QFT counterpart, the critical coupling. In addition, we provide a detailed overview of the calculation of exact anomalous dimensions and operator product expansion (OPE) coefficients in the conformal bi-scalar fishnet theory. The original contributions of this work comprise the results of the critical coupling for models with fermions, the brick wall theory, and the fermionic fishnet theory. Additionally, we extend the study of integrable Feynman graphs to supersymmetric diagrams in superspace. By establishing an efficient graphical formalism, we obtain the critical coupling of double-scaled $\beta$-deformations of $\mathcal{N} = 4$ super Yang-Mills theory and Aharony-Bergman-Jafferis-Maldacena theory, the super brick wall and superfishnet theory, respectively. Moreover, we apply superspace methods to the superfishnet theory and find results for anomalous dimensions and an OPE coefficient, which are all-loop exact in the coupling. In addition, we study boundary integrability in the six-vertex model and for Feynman diagrams. We present new box-shaped boundary conditions for the six-vertex model and conjecture a closed form for its partition function at any lattice size. On the QFT side, we find integrable boundary scattering matrices in the form of generalized Feynman diagrams by graphical methods.

==> packages/packages.tex <==

\usepackage[utf8]{inputenc} % Required for inputting international characters
\usepackage[T1]{fontenc} % Output font encoding for international characters
\usepackage{amsmath, amssymb, graphics}
\usepackage{lmodern} %font
\usepackage[english]{babel} % Required for automatically changing names of document elements to languages besides english
%\usepackage{cite}
\RequirePackage{scrbase} % Required for handling language-dependent names of sections/document elements
\RequirePackage{scrhack} % Loads fixes for various packages
\RequirePackage{setspace} % Required for changing line spacing
\RequirePackage{longtable} % Required for tables that span multiple pages (used in the symbols, abbreviations and physical constants pages)
\RequirePackage{siunitx} % Required for \SI commands
\RequirePackage{graphicx} % Required to include images
\graphicspath{{Figures/}{./}} % Specifies where to look for included images
\RequirePackage{booktabs} % Required for better table rules
\usepackage[margin=0cm, labelfont=bf]{caption} % Required for customising the captions
\usepackage{subcaption} % to use subfigure environment (pics side by side)

\usepackage{tensor}

\renewcommand\thefootnote{\textcolor{mypinegreen}{\arabic{footnote}}} %footnote color

\usepackage{etoolbox}
\patchcmd{\part}{\thispagestyle{plain}}{\thispagestyle{empty}}{}{}

%----------------------------------------------------------------------------------------
%	COLOURS
%----------------------------------------------------------------------------------------

\usepackage[dvipsnames]{xcolor} % Required for specifying custom colours
\definecolor{mypinegreen}{HTML}{083d89}

%----------------------------------------------------------------------------------------
%	ADDITIONAL PACKAGES
%----------------------------------------------------------------------------------------

\usepackage[autostyle=true]{csquotes} % Required to generate language-dependent quotes in the bibliography
\usepackage{verbatim} %to allow commenting sections
\usepackage{fancyhdr} %to use fancy as a style of the page
\usepackage{lipsum}
\usepackage[Sonny]{fncychap} %chapter style
\usepackage{amssymb,amsmath} %for formulas
\usepackage[nottoc]{tocbibind} %include references in the table of contents
\usepackage{hyperref}
\hypersetup{
    colorlinks=true,
    linkcolor=mypinegreen,          % color of internal links (change box color with linkbordercolor)
    citecolor=mypinegreen,
    filecolor=mypinegreen,      % color of file links
    urlcolor=mypinegreen
    }
\usepackage[numbered]{bookmark}
\usepackage{epsfig}
\usepackage{graphics, tikz}
\usepackage[multiple]{footmisc}
\usepackage{fancybox,framed,tikz}
\usetikzlibrary{decorations.pathmorphing,patterns}
\usepackage{dsfont}
\usepackage{mathtools} % for subequation numbering
\usepackage{braket} 
\usepackage{slashed} % for Feynman slashed notation
\usepackage{rotating}
\usepackage{bbold,amsfonts}
\usepackage{multirow}
\usepackage{upgreek}
\usepackage{amsfonts,euscript,amssymb,stmaryrd,braket}
\usetikzlibrary{shapes.misc,arrows,decorations.markings,patterns}
\usepackage{multirow}
\usepackage{tabularx}
\usepackage{bbold,bbding}
\usepackage{amsthm} 
\usepackage{esint}
\usepackage{simpler-wick} %for Wick contractions
\usepackage{tensor} % for typesetting mixed tensor indices
\usepackage{dsfont} % for displaying the blackboard 1 properly
\usetikzlibrary{positioning,arrows,calc}
\usetikzlibrary{arrows.meta}
\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{shapes.geometric}
\usetikzlibrary{patterns}
\usepackage{xparse}
\usepackage{diagbox} % for category cells in tables
\usepackage{tensor} % for typesetting mixed tensor indices
\usepackage{url} %to have urls with special characters
\usepackage{bibentry} %to cite fully paper in main text
%\usepackage[square,sort,comma,numbers]{natbib} %to make bibentry work
\usepackage[numbers,sort&compress]{natbib}
\usepackage{mathtools} %to write stuff over/under arrow

\usepackage{adjustbox} % \adjincludegraphics , aligns figures vertically in equations
\usepackage{mathrsfs}
%\usepackage{cellspace} % top and bottom space in tables with Sc or Sl Sr % \mathstrut in nominator is better
\usepackage{xfrac} % \sfrac

\usepackage[font={footnotesize}]{caption}

\newtheorem{theorem}{Theorem}

\tikzset{cross/.style={cross out, draw=black, minimum size=2*(#1-\pgflinewidth), inner sep=0pt, outer sep=0pt},
%default radius will be 1pt. 
cross/.default={1pt}}


